On Condorcet's Jury Theorem with Abstention

The well-known Condorcet Jury Theorem states that, under majority rule, the better of two alternatives is chosen with probability approaching one as the population grows. We study an asymmetric setting where voters face varying participation costs and share a possibly heuristic belief about their pivotality (ability to influence the outcome). In a costly voting setup where voters abstain if their participation cost is greater than their pivotality estimate, we identify a single property of the heuristic belief -- weakly vanishing pivotality -- that gives rise to multiple stable equilibria in which elections are nearly tied. In contrast, strongly vanishing pivotality (as in the standard Calculus of Voting model) yields a unique, trivial equilibrium where only zero-cost voters participate as the population grows. We then characterize when nontrivial equilibria satisfy a version of the Jury Theorem: below a sharp threshold, the majority-preferred candidate wins with probability approaching one; above it, both candidates either win with equal probability.

==> figures/nonlinear_support.tex <==
% \documentclass[11pt]{article}
% \usepackage{tikz}
% \usetikzlibrary{shapes.geometric, arrows, fit}
% \usetikzlibrary{decorations.pathreplacing}
% \begin{document}


%  \begin{figure}[ht!]
 %%%%%%%%%%%%
 \centering 
 \begin{tikzpicture}[scale=0.88]
\def\a{40}
\def\bx{-20}
\def\by{-13}
\draw[blue,thick] (0,1) -- (2,1.5) -- (4,3.5) -- (6,4) -- (8,4);
\draw[red,double] (0,0.5) -- (1.8,2.5) -- (5,3) -- (6.5,4) -- (7.3,4) --  (8,4.5);
\draw[thick,->] (0,0.3) -- (8,0.3);
\draw[dotted] (0.07,0.25) -- (0.07,2);
\node at (0.62,1.15) {$\circ$};
\draw[dashed] (0.62-0.1,0.5) -- (0.62-0.1,1.15+1);
\draw[dashed] (0.62+0.1,0.5) -- (0.62+0.1,1.15+1);
\node at (0.62-0.2,0) {$c^-_1$};
\node at (0.62+0.2,0) {$c^+_1$};


\node at (3.23,2.72) {$\circ$};
\draw[dashed] (3.23-0.3,0.5) -- (3.23-0.3,2.72+1);
\draw[dashed] (3.23+0.2, 0.5) -- (3.23+0.2,2.72+1);
\node at (3.23-0.3,0) {$c_2^-$};
\node at (3.23+0.2,0) {$c_2^+$};


\node at (6.5,4) {$\circ$};
\draw[dashed] (6.5-0.4,0.5) -- (6.5-0.4,4+1);
\node at (7.3,4) {$\circ$};
\node at (6.5-0.4,0) {$c_3^-$};

\draw[dashed] (7.3+0.3, 0.5) -- (7.3+0.3,4+1);
\node at (7.3+0.3,0) {$c_3^+$};


%\node at (0,-0.5) {$c=0$};
%\node at (8,-0.5) {$c=1$};





\node[blue] at (8.2,3.5) {$s_B$};

\node[red] at (8.2,4.8) {$s_A$};



% \tikzstyle{dot}=[rectangle,draw=black,fill=white,inner sep=0pt,minimum size=4mm]
% \tikzstyle{active}=[circle,draw=blue,fill=blue,inner sep=0pt,minimum size=2mm]
% \tikzstyle{inactive}=[circle,draw=blue,fill=white,inner sep=0pt,minimum size=2mm]
% \tikzstyle{sybil}=[rectangle,draw=black,fill=red,inner sep=0pt,minimum size=1.6mm]
% \tikzstyle{del}=[triangle,draw=blue,fill=white,inner sep=0pt,minimum size=2mm]
% \tikzstyle{virtual}=[diamond,draw=black,fill=gray,inner sep=0pt,minimum size=2mm]
% \tikzstyle{txt}=[text width = 8cm, anchor=west]

\end{tikzpicture}
  
%%%%%%%%%%%%%%%%%%
% %\includegraphics[width= 0.52 \textwidth]{Figure_3.png}
% \caption{A schematic illustration of equilibria points with piecewise linear support functions.  The dotted line marks the trivial equilibrium close to $c=0$. We can see there are two nontrivial equilibria on the sides of each intersection point/interval of the support functions.}
% \label{fig:nonlinear}
% \end{figure}

% \end{document}

